$f$-PO: Generalizing Preference Optimization with $f$-divergence Minimization

Preference optimization has made significant progress recently, with numerous methods developed to align language models with human preferences. This paper introduces $f$-divergence Preference Optimization ($f$-PO), a novel framework that generalizes and extends existing approaches. $f$-PO minimizes $f$-divergences between the optimized policy and the optimal policy, encompassing a broad family of alignment methods using various divergences. Our approach unifies previous algorithms like DPO and EXO, while offering new variants through different choices of $f$-divergences. We provide theoretical analysis of $f$-PO's properties and conduct extensive experiments on state-of-the-art language models using benchmark datasets. Results demonstrate $f$-PO's effectiveness across various tasks, achieving superior performance compared to existing methods on popular benchmarks such as AlpacaEval 2, Arena-Hard, MT-Bench, and Open LLM Leaderboard v2. Additionally, we present ablation studies exploring the impact of different $f$-divergences, offering insights into the trade-offs between regularization and performance in offline preference optimization. Our work contributes both practical algorithms and theoretical understanding to the field of language model alignment. Code is available at https://github.com/MinkaiXu/fPO.

==> tables/hyperparams_baselines.tex <==

% \setlength{\tabcolsep}{4pt}
\begin{table*}[!h]
\vspace{-1em}
\caption{Various preference optimization objectives and hyperparameter search range.}
\label{tab:hyperparams_baseline}
\centering
\resizebox{\textwidth}{!}{
\small
\begin{tabular}{lll}
\toprule 
\textbf{Method} & \textbf{Objective} & \textbf{Hyperparameter} \\ \midrule
% \midrule 
RRHF~\cite{yuan2023rrhf} & $\max \left(0, - \frac{1}{|y_w|} \log \pi_\theta(y_w|x) + \frac{1}{|y_l|} \log \pi_\theta(y_l|x)\right) - \lambda \log \pi_\theta (y_w | x)$ & $\lambda \in [0.1, 0.5, 1.0, 10.0]$ \\ \midrule 
\multirow{2}{*}{SLiC-HF~\cite{Zhao2023SLiCHFSL}} & \multirow{2}{*}{$\max\left(0, \delta - \log \pi_\theta(y_w|x) + \log \pi_\theta(y_l|x)\right) - \lambda \log \pi_\theta (y_w | x)$} & $\lambda \in [0.1, 0.5, 1.0, 10.0]$ \\
&  & $\beta \in [0.1, 0.5, 1.0, 2.0]$ \\
\midrule 
DPO~\cite{rafailov2023direct} & $-\log \sigma \left( \beta \log \frac{\pi_\theta(y_w|x)}{\pi_{\text{ref}}(y_w|x)} - \beta \log \frac{\pi_\theta(y_l|x)}{\pi_{\text{ref}}(y_l|x)}\right)$ & $\beta \in [0.01, 0.05, 0.1]$ \\ \midrule 
IPO~\cite{Azar2023AGT} & $ \left( \log \frac{\pi_\theta(y_w|x)}{\pi_{\text{ref}}(y_w|x)} - \log \frac{\pi_\theta(y_l|x)}{\pi_{\text{ref}}(y_l|x)} - \frac{1}{2\tau} \right)^2$ & $\tau \in [0.01, 0.1, 0.5, 1.0]$ \\  \midrule 
CPO~\cite{xu2024contrastive} &  $-\log \sigma  \left(\beta \log \pi_\theta(y_w|x) - \beta \log \pi_\theta(y_l|x) \right) - \lambda \log \pi_\theta (y_w|x)$ & $\alpha = 1.0, \,\, \beta \in [0.01, 0.05, 0.1]$ \\ \midrule
\multirow{2}{*}{KTO~\cite{Ethayarajh2024KTOMA}} & $-\lambda_w \sigma \left( \beta \log \frac{\pi_\theta(y_w|x)}{\pi_{\text{ref}}(y_w|x)} - z_{\text{ref}} \right) +  \lambda_l \sigma \left( z_{\text{ref}} - \beta \log \frac{\pi_\theta(y_l|x)}{\pi_{\text{ref}}(y_l|x)} \right),\,$ & $\lambda_l = \lambda_w = 1.0$ \\  
& $\text{where} \,\, z_{\text{ref}} = \mathbb{E}_{(x, y) \sim \mathcal{D}} \left[\beta \text{KL}\left( \pi_\theta(y|x) || \pi_{\text{ref}}(y|x) \right)  \right]$ & $\beta \in [0.01, 0.05, 0.1]$ \\ \midrule
\multirow{2}{*}{ORPO~\cite{Hong2024ORPOMP}} & $-\log p_\theta(y_w|x) - \lambda  \log \sigma \left(\log \frac{p_\theta(y_w|x)}{1 - p_\theta(y_w|x)} - \log \frac{p_\theta(y_l|x)}{1 - p_\theta(y_l|x)}  \right),\,$ & \multirow{2}{*}{$\lambda \in [0.1, 0.5, 1.0, 2.0]$} \\  
& $\text{where} \,\, p_\theta(y|x) = \exp\left( \frac{1}{|y|} \log \pi_\theta(y|x) \right)$ \\  \midrule
\multirow{2}{*}{R-DPO~\cite{Park2024DisentanglingLF}} & \multirow{2}{*}{$-\log \sigma \left( \beta \log \frac{\pi_\theta(y_w|x)}{\pi_{\text{ref}}(y_w|x)} - \beta \log \frac{\pi_\theta(y_l|x)}{\pi_{\text{ref}}(y_l|x)} - \left(\alpha |y_w| - \alpha |y_l| \right) \right)$} & $\alpha \in [0.05, 0.1, 0.5, 1.0]$ \\
& & $\beta \in [0.01, 0.05, 0.1]$ \\
% \midrule 
% \multirow{2}{*}{EXO~\citep{ji2024towards}} & \multirow{2}{*}{} & $\beta \in [2.0, 2.5]$ \\
% & & $\gamma \in [0.3, 0.5, 1.0, 1.2, 1.4, 1.6]$ \\ 
\midrule 
\multirow{2}{*}{SimPO~\citep{meng2024simpo}} & \multirow{2}{*}{$-\log \sigma  \left( \frac{\beta}{|y_w|} \log \pi_\theta(y_w|x) - \frac{\beta}{|y_l|} \log \pi_\theta(y_l|x) - \gamma \right)$} & $\beta \in [2.0, 2.5]$ \\
& & $\gamma \in [0.3, 0.5, 1.0, 1.2, 1.4, 1.6]$ \\
\midrule 
\multirow{3}{*}{$f$-PO} & \multirow{3}{*}{} & $\beta \in [2.0, 2.5]$ \\
& & $\gamma \in [0.3, 0.5, 1.0, 1.2, 1.4, 1.6]$ \\ 
& & $\alpha \in []$ \\

\bottomrule
\end{tabular}
}
\end{table*}

==> tables/hyperparams_simpo.tex <==

% \setlength{\tabcolsep}{4pt}
% \begin{table*}[!t]
\begin{wraptable}[9]{r}{8.5cm}
\vspace{-1.3em}
\caption{The hyperparameter values in \methodabbrv used for each training setting.}
\label{tab:hyperparams_simpo}
\centering
% \resizebox{\textwidth}{!}{
\small
\begin{tabular}{lccccc}
\toprule 
\textbf{Setting} & $\alpha$ & $\beta$ & $\gamma$ & Learning rate \\ \midrule
\textbf{Mistral-Base} & 0.99 & 2.0 & 1.6 & 3e-7 \\
\textbf{Mistral-Instruct} & 0.925 & 2.5 & 0.3 & 6e-7 \\
\textbf{Llama3-Base} & 0.99 & 2.0 & 1.0 & 7e-7 \\
\textbf{Llama3-Instruct} & 0.99 & 2.6 & 1.43 & 1e-6 \\
\bottomrule
\end{tabular}
% }
\end{wraptable}
